Learning by Doing: The Case of Online Lending

Online lending, a phenomenon which is becoming mainstream due to the migration of consumer finance to the Internet and the adoption of AI based lending models, is an example of learning by doing. This paper studies optimal policies for a direct online lender. This is an instance of a more general problem: how should a decision-maker experiment sequentially in the face of unknown customer (or other) information? Conventional wisdom suggests the decision-maker should take advantage of sequential learning opportunities by conducting multiple small, lean experiments, each building incrementally on the results of earlier ones. Can a single grand experiment, uninformed by earlier experiments, do as well? We find that lean incremental experiments are optimal when the interest rate is exogenous. However, when we extend the lender's action space to setting both the interest rate and the loan amount, we find conditions under which a single grand experiment is optimal. In both cases, income variability can benefit the lender by enabling more effective experimentation. We also study the consumer segmentation associated with each strategy and show that the lender cannot achieve more than half the profit obtained under perfect information.

==> Proof/Proof_worst_case.tex <==
\subsection{Proof of Proposition \ref{worstcase}}
\label{app_worstcase}
First, the following lemma to guarantee under optimal policy, the online lenders return is strictly positive for any distribution with fixed mean $l>0$.

\begin{lemma}
\label{positive_return}
For any distribution with fixed mean $l>0$, there exists $\epsilon>0$ such that the online lender's expected profit $\Pi\geq\epsilon>0$.
\end{lemma}

To prove this, simply notice that in exogenous interest rate, for any $d$, the online lender's expected profit is lower bounded by 
\myeql{
\tilde{\Pi}=\max_{y}  - dy+\rho (1-F(y))\left(\dfrac{(1-d)y}{(1-\rho)}\right)
}

At $y=0$, the derivative of $\tilde{\Pi}$ becomes
\myeql{
\dfrac{\partial \tilde{\Pi}}{\partial \mu}|_{y=0}=-d+\dfrac{\rho (1-d) }{(1-\rho)}>0
}

In endogenous interest rate, for any $d\in(0,\rho)$, one have the online lender's expected profit is lowerbounded by
\myeql{
\tilde{\Pi}=\max_{y}  - s(d)d y+\rho s(d) (1-F(y))\dfrac{(1-d^{\alpha+1})}{(1-d^{\alpha}\rho)}y
}

At $y=0$, the derivative of $\tilde{\Pi}$ becomes
\myeql{
\dfrac{\partial \tilde{\Pi}}{\partial \mu}|_{y=0}=-s(d) d+\rho s(d)\dfrac{ (1-d^{\alpha+1}) }{(1-d^{\alpha}\rho)}>0
}
Hence when $y=0$, $\tilde{\Pi}=0$, which implies that $\tilde{\Pi}$ under optimal policy is strictly greater than $0$. There exists $\epsilon$ such that $\tilde{\Pi}\geq\epsilon>0$, which implies the expected return of $\Pi(F\in\mathcal{F})\geq \epsilon>0$, where $\Pi(F\in\mathcal{F})$ is the online lender's expected return under optimal policy with income distribution $F$ in the class of distribution, and $F$ has a twice continuously differentiable density function $f$ defined over the continuous positive support $[0,u)$. 

Now we show that  if there exists $\lambda(\epsilon)$ such that for all $\epsilon>0$ (1) $\int^{\infty}_0xdF_{\lambda(\epsilon)}(x)=l$, and (2) $\epsilon H_{\lambda(\epsilon)}(\epsilon)\geq1$, the expected profit goes to $0$. To prove this, simply notice that  $\epsilon H_{\lambda(\epsilon)}(\epsilon)\geq1$ implies $\bar{x}<\epsilon$. Note that the online lender's expected return is upper bounded by $\frac{\rho-d}{1-\rho}\bar{x}$ in exogenous interest rate and $\rho (d^*)^{\alpha}\frac{1-(d^*)^{\alpha+1}}{1-(d^*)^{\alpha}\rho}\bar{x}$. As $\bar{x}$ goes to $0$, the expected profit also goes to $0$.

We now construct a distribution that provides the online lender with expected payoff arbitrarily close to $0$. Note under both cases, 
$$G(x)=\delta \in (0, 1)$$
in exogenous distribution $\delta =  \frac{(\rho -d) }{\rho(1-d)} $, In endogenous distribution with constant elasticity $\delta = \frac{1}{\alpha+1}$, with decreasing and increasing elasticity, $\delta=-\frac{(1-\rho s(d^*))}{(1-s(d^*)d^*)}\frac{d^*}{\rho}+1\in(0,1)$ following lemma \ref{lemma_general_barx_dr_1}.

Consider the Lomax distribution positively support in $[0,\infty)$ with parameters $a$ and $\lambda$.
$$f(x)=\frac{a}{\lambda}\left(1+\frac{x}{\lambda}\right)^{-(a+1)}, \quad F(x)=1-\left(1+\frac{x}{\lambda}\right)^{-a}$$
$G(x)$ is given by
$$G(x)=\dfrac{a }{\lambda/x+1}$$
and $G(x)$ is monotone increasing.

Note the mean of Lomax distribution is given by
$\frac{\lambda}{a-1}$ for $a >1$. Set $a = \frac{\lambda}{l}+1$ would control the mean to be $l$, and 
$$G(\bar{x}) = \frac{\lambda/l+1}{\lambda/x+1}$$
Hence 
$$\bar{x}=\dfrac{\delta  \lambda}{\lambda/l + 1-\delta }$$
For any fixed $l$, $\delta\in(0,1)$, as $\lambda$ goes to $0$, $\bar{x}$ also goes to $0$, hence there exists distribution such that $\bar{x}$ is arbitrarily close to $0$. 
